Eagle: Efficient Training-Free Router for Multi-LLM Inference

The proliferation of Large Language Models (LLMs) with varying capabilities and costs has created a need for efficient model selection in AI systems. LLM routers address this need by dynamically choosing the most suitable model for a given query based on task requirements and budget constraints. However, existing routers face challenges in scalability and real-time adaptation, particularly in high-volume online environments. We present Eagle, a novel LLM routing approach that combines global and local ELO ranking modules to overcome these limitations. By evaluating both general and specialized LLM abilities, Eagle provides a scalable, training-free solution that enhances model selection quality while reducing computational overhead. Our experiments across multiple datasets show Eagle consistently outperforms baseline methods, with improvements of up to 23.52 percent in Area Under Curve (AUC) scores. Moreover, Eagle demonstrates remarkable efficiency, requiring only 1/20 of baseline methods' time for initialization and 100 to 200 times faster incremental updates in online scenarios, making it well-suited for dynamic, high-volume online serving environments.

==> prompts.tex <==

\definecolor{teal}{RGB}{0, 128, 128} %
\definecolor{myblue}{RGB}{79, 129, 189} %



\tcbset{
  colback=teal!10!white,
  colframe=teal!20,
  coltitle=black,
  left=4mm,
  right=4mm,
  boxsep=5mm,
  arc=2mm,
  box align=top,
  halign=left, %
  title filled=false,
  center title, %
  fonttitle=\bfseries
}




\newcommand{\myprompt}[3]{
  \begin{tcolorbox}[title=#1]
  #2
  \end{tcolorbox}
}


\definecolor{boxbackground}{RGB}{255,255,255} %
\definecolor{boxframe}{RGB}{0,0,0} %

\tcbset{
  myprompt/.style={
    colback=boxbackground, %
    colframe=boxframe, %
    coltitle=boxframe, %
    fonttitle=\bfseries, %
    sharp corners, %
    detach title, %
    before upper={\tcbtitle\par\medskip}, %
    fontupper=\normalsize, %
    toprule=1pt, %
    bottomrule=1pt, %
    leftrule=1pt, %
    rightrule=1pt, %
    boxsep=5pt, %
    arc=0pt, %
    outer arc=0pt, %
    box align=top, %
    halign=left, %
    breakable, %
    enhanced jigsaw, %
  }
}

\newcommand{\nodeprompt}[4]{
  \begin{tcolorbox}[myprompt, title=Prompt Box]
    \textbf{Question:} #1
    
    \textbf{Complete Outline:} #2
    
    \textbf{Current Node (Node #3):} ``#4''
    
    \textbf{Context from Previous Nodes:}
    #2 %
    
    \textbf{Instructions:}
    \begin{itemize}[leftmargin=*]
      \item Craft a response that is tightly focused on the topic of ``#4''. If this node depends on earlier ones, weave in relevant details from those nodes to enrich your explanation.
      \item Keep your response between 1-5 sentences to maintain conciseness without sacrificing depth or insight.
      \item Directly address the specifics of the node, avoiding broad generalizations or unrelated information.
    \end{itemize}
    
    \textbf{Response:}
  \end{tcolorbox}
}


\tcbset{
  myprompt2/.style={
    colback=boxbackground, %
    colframe=boxframe, %
    coltitle=boxframe, %
    fonttitle=\bfseries, %
    sharp corners, %
    detach title, %
    before upper={\tcbtitle\par\medskip}, %
    fontupper=\normalsize, %
    toprule=1pt, %
    bottomrule=1pt, %
    leftrule=1pt, %
    rightrule=1pt, %
    boxsep=5pt, %
    arc=0pt, %
    outer arc=0pt, %
    box align=top, %
    halign=left, %
    breakable, %
    enhanced jigsaw, %
  }
}

\newcommand{\skeletonprompt}[1]{
  \begin{tcolorbox}[myprompt2, title=Structured Outline Prompt]
    Create a structured outline for a specific question: \textbf{#1} by following these steps:
    \begin{enumerate}[leftmargin=*]
      \item Format the answer as an outline with 1-8 main points, each described as follows:
      \begin{itemize}
        \item \texttt{Node('Brief description', previous=[Dependent Nodes], knowledgeLevel=1-10)}
        \begin{itemize}
          \item ``\texttt{knowledgeLevel=1-4}'' indicates a point requiring common sense or general knowledge.
          \item ``\texttt{knowledgeLevel=5}'' serves as a midpoint, indicating a balance between common knowledge and more specialized reasoning.
          \item ``\texttt{knowledgeLevel=6-10}'' indicates a point requiring logical reasoning, mathematical computation, and specialized knowledge.
        \end{itemize}
      \end{itemize}
    \end{enumerate}
    
    \textbf{Guidelines:}
    \begin{itemize}[leftmargin=*]
      \item Aim for conciseness and logical sequence.
      \item Combine simpler steps to reduce the total number of nodes.
      \item Ensure each node includes dependencies and a knowledge level rating.
      \item Only output the nodes without additional information.
    \end{itemize}
    
    \textbf{Examples:}
    \begin{itemize}[leftmargin=*]
      \item How to prepare for a marathon?:
      \begin{itemize}
        \item \texttt{Node('Establish a training schedule', previous=[], knowledgeLevel=3)}
        \item \texttt{Node('Choose the right gear', previous=[], knowledgeLevel=4)}
        \item \texttt{Node('Incorporate cross-training', previous=[], knowledgeLevel=5)}
        \item \texttt{Node('Plan nutrition and hydration', previous=[], knowledgeLevel=7)}
        \item \texttt{Node('Build up mileage gradually', previous=[1], knowledgeLevel=5)}
        \item \texttt{Node('Taper before the race', previous=[1,4], knowledgeLevel=6)}
      \end{itemize}
      \item How to find the roots of a quadratic equation \( ax^2 + bx + c = 0 \)?:
      \begin{itemize}
        \item \texttt{Node('Understand the quadratic formula', previous=[], knowledgeLevel=5)}
        \item \texttt{Node('Identify coefficients and calculate the discriminant', previous=[1], knowledgeLevel=6)}
        \item \texttt{Node('Apply the formula and solve for x', previous=[2], knowledgeLevel=7)}
    \end{itemize}

    The goal is to provide a clear, actionable outline that serves as a roadmap for answering the question, using as few nodes as possible.

    
  \end{tcolorbox}
}

